Formalizing Statistical Causality via Modal Logic

We propose a formal language for describing and explaining statistical causality. Concretely, we define Statistical Causality Language (StaCL) for expressing causal effects and specifying the requirements for causal inference. StaCL incorporates modal operators for interventions to express causal properties between probability distributions in different possible worlds in a Kripke model. We formalize axioms for probability distributions, interventions, and causal predicates using StaCL formulas. These axioms are expressive enough to derive the rules of Pearl's do-calculus. Finally, we demonstrate by examples that StaCL can be used to specify and explain the correctness of statistical causal inference.

==> _axioms-AX-CP-G.tex <==

\begin{figure}[t]
\centering
\begin{screen}[7]
\begin{small}
\begin{flushleft}
\[
\renewcommand{\arraystretch}{1.20}
\begin{array}{@{\hspace{-1.0ex}}l@{\hspace{-0.5ex}}l}
\phantom{\mbox{\axXpdEL{}}}~&~~
\\[-4.5ex]
\!\mbox{\axDGEq}
&~~~ \vdashGG \bmx = \bmu
~\,\mbox{ if } \datagenerator(\bmx) = \bmu
\\
\!\mbox{\axDsepDG{}}
&~~~ \vdashGG \dsep(\bmx, \bmy, \bmz)
~~~ \mbox{if } \modelsg \dsep(\bmx, \bmy, \bmz)
\hspace{3ex}~
\\
\!\mbox{\axNancDG{}\hspace{1ex}}
&~~~ \vdashGG \nanc(\bmx, \bmy)
~~~ \mbox{if } \modelsg \nanc(\bmx, \bmy)
~\hspace{25.0ex}~
\\
\end{array}
\]
\end{flushleft}
\end{small}
\end{screen}
\caption{The additional axioms for \AXwGCP{} for
disjoint $\bmx, \bmy, \bmz$ 
and
$\bmu \in \Term^+$.}
\label{fig:AXGCP}
\end{figure}

